Quantile Granger Causality in the Presence of Instability

We propose a new framework for assessing Granger causality in quantiles in unstable environments, for a fixed quantile or over a continuum of quantile levels. Our proposed test statistics are consistent against fixed alternatives, they have nontrivial power against local alternatives, and they are pivotal in certain important special cases. In addition, we show the validity of a bootstrap procedure when asymptotic distributions depend on nuisance parameters. Monte Carlo simulations reveal that the proposed test statistics have correct empirical size and high power, even in absence of structural breaks. Moreover, a procedure providing additional insight into the timing of Granger causal regimes based on our new tests is proposed. Finally, an empirical application in energy economics highlights the applicability of our method as the new tests provide stronger evidence of Granger causality.

==> old/lemA1_old.tex <==
% {\bf Proof sketches at given $\tau \in (0,1)$}

% Because
% \[
% {\sf J}^{-1/2}{\sf H} \begin{bmatrix} 0_{p \times p} & 0_{p \times k} \\  0_{k \times p} & {\sf H}_{22}^{-1}({\sf J}_{22}^{-1/2})^{-1} \end{bmatrix} =\begin{bmatrix} 0_{p \times p} & 0_{p \times k} \\  0_{k \times p} & I_k \end{bmatrix}
% \]
% we get
% \begin{align*}
% {\sf J}^{-1/2}{\sf H}\sqrt{n}(\tilde\beta_n(\tau)-\beta_0(\tau)) = \,&-{\sf J}^{-1/2}{\sf H}\begin{bmatrix} 0_p \\ {\sf H}_{22}^{-1}S_{n,2}(1,\tau,\beta_{2,0}(\tau)) \end{bmatrix} + o_p(1) \\
% % = \,& -\frac{{\sf J}^{-1/2}{\sf H}}{\tau(1-\tau)} \begin{bmatrix} 0_{p \times p} & 0_{p \times k} \\  0_{k \times p} & {\sf H}_{22}^{-1}({\sf J}_{22}^{-1/2})^{-1} \end{bmatrix} \begin{bmatrix} 0_p \\ {\sf J}_{22}^{-1/2}S_{2,n}(1,\tau,\beta_0(\tau)) \end{bmatrix} + o_p(1) \\
% = \,& - \begin{bmatrix} 0_p \\ {\sf J}_{22}^{-1/2}S_{2,n}(1,\tau,\beta_{2,0}(\tau)) \end{bmatrix} + o_p(1)
% \end{align*}

Now, let $\beta_{i,n} \coloneqq (\beta_{1,i,n}',\beta_{2,0}')'$, and consider
\begin{align*}
  S_{n,2}(1,\tau,\beta_{2,0}) = \,& \frac{1}{\sqrt n}\sum_{i=1}^n x_{2,i} \psi_\tau(y_i-x_{2,i}'\beta_{2,0}) \\
  = \,& \frac{1}{\sqrt n}\sum_{i=1}^n x_{2,i} \psi_\tau(y_i-x_i'\beta_{i,n}) \\
  \,& +  \frac{1}{\sqrt n}\sum_{i=1}^n x_{2,i} \big[1\{y_i \leq x_{2,i}'\beta_{2,0}\}  -1\{y_i\leq x_i'\beta_{i,n}\} - F_i(x_{2,i}'\beta_{2,0})+F_i(x_{i}'\beta_{i,
n})\big] \\
\,& + \frac1{\sqrt n} \sum_{i=1}^n x_{2,i} (F_i(x_i'\beta_{i,n})-F_i(x_{2,i}'\beta_{2,0})) \eqqcolon A + B +C.
\end{align*}
We know that ($1$) $(\tau(1-\tau){\sf J_{22}})^{-1/2}A \rightarrow_d {\cal B}_k(1)$, ($2$) by stochastic equicontinuity $B = o_p(1)$, while, using a Taylor-series expansion
\begin{align*}
C =  \,& \frac{1}{n}\sum_{i=1}^n x_{2,i}x_{1,i}'f_i(x_i'\beta_{i,n})\beta_{1,i,n}+o_p(1) \\
  = \,& \frac{1}{n}\sum_{i=1}^n x_{2,i}x_{1,i}'f_i(x_i'\beta_{i,n})(\Delta_1(\tau)+\Delta_2(\tau)g(i/n)) + o_p(1) \\
   \,&  \rightarrow_p {\sf H}_{21}(\Delta(\tau)+\delta(\tau)\int_0^1g(v){\sf d}v)\end{align*}
with
\[
c(\tau,\lambda) \coloneqq \Delta_1(\tau)+\Delta_2(\tau)\int_{0}^{\lambda}g(v){\sf d}v.
\]
 Therefore,
 \[
 (\tau(1-\tau){\sf J})^{-1/2}{\sf H}\sqrt{n}(\tilde\beta_n(\tau)-\beta_0(\tau)) \rightarrow_d \begin{bmatrix}
     0_p \\ (\tau(1-\tau){\sf J}_{22})^{-1/2}{\sf H}_{12}c(\tau)+{\cal B}_k(1).
 \end{bmatrix}
 \]
 Similarly, 
 \begin{align*}
 S_n(\lambda,\tau,\beta_0(\tau)) = \,& \frac1{\sqrt n}\sum_{i=1}^{\floor{\lambda n}} x_{i} \psi_\tau(y_i-x_i'\beta_{i,n}) \\
 \,& + \frac1{\sqrt n}\sum_{i=1}^{\floor{\lambda n}} x_i\left[F_i(x_i'\beta_{i,n})-F_i(x_{2,i}'\beta_{2,0}) \right] + o_p(1).
 \end{align*}
 Now,
 \[
 (\tau(1-\tau){\sf J})^{-1/2}\frac1{\sqrt n}\sum_{i=1}^{\floor{\lambda n}} x_{i} \psi_\tau(y_i-x_i'\beta_{i,n}) \Rightarrow {\cal B}_m(\lambda)
 \]

\[
\frac1{\sqrt n}\sum_{i=1}^{\floor{\lambda n}} x_ix_i'f_i(x_i'\beta_{i,n})\bar{R}\beta_{1,i,n}(\tau) \rightarrow_p \lambda {\sf H}\bar{R}\Delta(\tau)+\delta(\tau){\sf H}\bar{R}\int_0^\lambda g(v){\sf d}v, \quad \bar{R} \coloneqq \begin{bmatrix} I_p \\ 0_{k\times p} \end{bmatrix}
\]

 Thus,
 \[
  (\tau(1-\tau){\sf J})^{-1/2}S_n(\lambda,\tau,\beta_0(\tau)) \Rightarrow {\cal B}_m(\lambda) + \lambda  (\tau(1-\tau){\sf J})^{-1/2}{\sf H}\bar{R}c(\tau,\lambda)
 \]


 \[
 {\sf J}^{-1/2}{\sf H}\bar R c(\tau,\lambda)-R{\sf J_{22}}^{-1/2}{\sf H_{21}}c(\tau,1)
 \]

 % \[
 % \lambda c(\tau,\lambda)-\lambda c(\tau,) = \Delta_2(\tau)\left(\int_0^\lambda g(v){\sf d}v-\lambda\int_0^1 g(v){\sf d}v\right)
 % \]

  Thus,
 \begin{align*}
     {\sf J}^{-1/2}S_n(\lambda,\tau,\tilde\beta_n(\tau)) \Rightarrow \begin{bmatrix} {\mathcal B}_p(\lambda) \\ {\cal BB}_k(\lambda) \end{bmatrix} + \lambda \Xi(\tau,\lambda)
 \end{align*}
where, with $\bar M \coloneqq I_m-M$, we have
\begin{align*}
\Xi(\tau,\lambda) \coloneqq \,& {\sf J}^{-1/2}{\sf H}\bar{R}c(\tau,\lambda)-\bar M {\sf J}^{-1/2}{\sf H}\bar{R}c(\tau,1) \\
= \,& {\sf J}^{-1/2}{\sf H}\bar{R}\Delta(\tau)-\bar M {\sf J}^{-1/2}{\sf H}\bar{R}\Delta(\tau) \\
\,&+ {\sf J}^{-1/2}{\sf H}\bar{R}\delta(\tau)\int_0^\lambda g(v){\sf d}v-\bar M {\sf J}^{-1/2}{\sf H}\bar{R}\delta(\tau)\int_0^1 g(v){\sf d}v 
\eqqcolon  \Xi_1(\tau)+\Xi_2(\tau,\lambda).
\end{align*}
Some manipulations reveal,
\begin{align*}
    \Xi_1(\tau) = \begin{bmatrix} \bar R'{\sf J}^{-1/2}{\sf H}\bar{R}\Delta(\tau) \\ 0_k\end{bmatrix} \quad
    \Xi_2(\tau) = \delta(\tau)\begin{bmatrix} \bar R'{\sf J}^{-1/2}{\sf H}\bar{R}\int_0^\lambda g(v){\sf d}v \\ -R'{\sf J}^{-1/2}{\sf H}\bar{R}\int_\lambda^1 g(v){\sf d}v \end{bmatrix} 
\end{align*}

Hence,
\begin{align*}
    H_n(1,\tau,\tilde\beta_n(\tau)) \rightarrow_d {\cal B}_p(1)+ \bar R'{\sf J}^{-1/2}{\sf H}\bar{R}(\Delta(\tau)+\delta(\tau)\int_0^1 g(v){\sf d}v).
\end{align*}
and
\begin{align*}
    \tilde H_n(\lambda,\tau,\tilde\beta_n(\tau))\bar R \Rightarrow {\cal B}{\cal B}_p(\lambda) -\delta(\tau)\bar R'{\sf J}^{-1/2}{\sf H}\bar{R}\int_\lambda^1 g(v){\sf d}v
\end{align*}

==> old/oldproof.tex <==
\textbf{Proof of Proposition \ref{prop1}.}  Let $\tilde\beta_{2,n}(\tau)$ be the solution to the constrained optimization defined in Eq. \eqref{eq:beta_tilde} (assuming $\beta_{1}(\tau) = 0$).  Moreover, set
\[
R  \coloneqq \begin{bmatrix}
    0_{p \times k} \\  I_k
\end{bmatrix},
\]
so that 
\[
R\beta_{2,0}(\tau) = \tilde\beta_0(\tau) \coloneqq \begin{bmatrix}
    0_p \\ \beta_{2,0}(\tau)
\end{bmatrix}.
\]
Define also \({\sf Q} \coloneqq \Ex[x_ix_i']\),  $s(\tau) = 1/f(F^{-1}(\tau))$. The following is based on \citet[Proof of Lemma 1]{qu:2008}: Under the null of $\beta_{1,0}(\tau) = 0$
\begin{align*}
S_n(\lambda,\tau,\tilde\beta_n(\tau))= \,& S_n(\lambda,\tau,\tilde\beta_0(\tau)) + \frac{1}{\sqrt{n}}\sum_{i=1}^{\floor{\lambda n}}x_i(F_i(x_{2,i}'\beta_{2,n})-\tau) + o_p(1)\\
\stackrel{(1)}{=} \,& S_n(\lambda,\tau,\beta_0(\tau)) + \frac{1}{n}\sum_{i=1}^{\floor{\lambda n}}x_ix_{2,i}' f_i(x_{2,i}'\beta_{2,0}(\tau))\sqrt{n}(\beta_{2,n}(\tau)-\beta_{2,0}(\tau)) + o_p(1)\\
\stackrel{(2)}{=} \,& S_n(\lambda,\tau,\beta_0(\tau)) + \frac{1}{n}\sum_{i=1}^{\floor{\lambda n}}x_ix_i'f_i(x_i'\beta_0(\tau)) (R \sqrt{n}(\beta_{2,n}(\tau)-\beta_{2,0}(\tau)))  + o_p(1) \\
\stackrel{(3)}{=} \,& S_n(\lambda,\tau,\beta_0(\tau)) +  \frac{\lambda}{s(\tau)} {\sf Q}\sqrt{n}(\tilde\beta_n(\tau)-\beta_0(\tau)) + o_p(1), \quad \tilde\beta_n(\tau) = (0,\tilde\beta_{2,n}'(\tau))', 
\end{align*}
where (1) uses a mean-value expansion, (2) is due to $x_ix_i'R = x_ix_{2,i}'$ and (3) is based on $n^{-1}\sum_{i=1}^{\floor{\lambda n}}x_ix_i'f_i(x_i'\beta_0(\tau)) = \lambda {\sf Q}/s(\tau) + o_p(1).$ Moreover, let ${\sf Q}_{ij}$, $i,j \in \{1,2\}$, denote the $ij$-th block of ${\sf Q}$ and partition 
\[
S_n(\lambda,\tau,t) = (S_{1,n}(\lambda,\tau,t)',S_{2,n}(\lambda,\tau,t)')'
\]
to conform with $\beta_0(\tau) = (\beta_{1,0}(\tau)',\beta_{2,0}(\tau)')'$. Then,
\[
\sqrt{n}(\tilde\beta_n(\tau)-\beta_0(\tau)) = -s(\tau)\begin{bmatrix} 0_p \\ {\sf Q}_{22}^{-1}S_{n,2}(1,\tau,\beta_0(\tau)) \end{bmatrix} + o_p(1),
\]
see also \citet[Proof of Thm 1]{koemach:99} for the partitioning. Next, note that
\[
(\tau(1-\tau){\sf Q})^{-1/2}S_{n}(\lambda,\tau,\theta_0(\tau))  \Rightarrow {\cal B}_{m}(\lambda) 
\]
and
\begin{align*}
    (\tau(1-\tau){\sf Q}_{22})^{-1/2}&S_{2,n}(\lambda,\tau,\theta_0(\tau))  \\
    = & (\tau(1-\tau){\sf Q}_{22})^{-1/2}\frac{1}{\sqrt{n}}\sum_{i=1}^{\floor{\lambda n}} x_{2,i}\psi_{\tau}(y_i-x_{2,i}'\beta_2(\tau))  \Rightarrow {\cal B}_k(\lambda). 
\end{align*}
Therefore, 
\begin{align*}
\begin{bmatrix} 0_p \\ {\sf Q}_{22}^{-1}S_{n,2}(1,\tau,\beta_0(\tau)) \end{bmatrix} 
% = \,&
% \begin{bmatrix} 0_p \\ {\sf Q}_{22}^{-1}({\sf Q}_{22}^{-1/2})^{-1}{\sf Q}_{22}^{-1/2}S_{n,2}(1,\tau,\beta_0(\tau)) \end{bmatrix} \\
= \,& \begin{bmatrix} 0_{p \times p} & 0_{p \times k} \\  0_{k \times p} & {\sf Q}_{22}^{-1}({\sf Q}_{22}^{-1/2})^{-1} \end{bmatrix} \begin{bmatrix} 0_p \\ {\sf Q}_{22}^{-1/2}S_{n,2}(1,\tau,\beta_0(\tau)) \end{bmatrix}
\end{align*}
Because, 
\[
{\sf Q}^{-1/2}{\sf Q} \begin{bmatrix} 0_{p \times p} & 0_{p \times k} \\  0_{k \times p} & {\sf Q}_{22}^{-1}({\sf Q}_{22}^{-1/2})^{-1} \end{bmatrix} =\begin{bmatrix} 0_{p \times p} & 0_{p \times k} \\  0_{k \times p} & I_k \end{bmatrix}
\]
and $X'X/n = {\sf Q} + o_p(1)$, the claim follows. \hfill$\square$

\textbf{Proof of Corollary \ref{cor1}.} By Proposition \ref{prop1},
$\tilde H_n(\lambda,\tau,\tilde\beta_n(\tau))\Rightarrow \sqrt{\tau(1-\tau)} {\cal{BB}}_{m}(\lambda),$ so that
\[
\tilde H_n(\lambda,\tau,\tilde\beta_n(\tau))M \Rightarrow \sqrt{\tau(1-\tau)}\begin{bmatrix} {\mathcal{BB}_p}(\lambda) \\ 0_k \end{bmatrix},
\]
and, because $\mathcal{BB}(1)=0$,
\[
H_n(1,\tau,\tilde\beta_n(\tau)) \Rightarrow \sqrt{\tau(1-\tau)}\begin{bmatrix} {\mathcal{B}_p}(1) \\ 0_k \end{bmatrix}
\]
The claim follows from the continuous mapping theorem noting that $\mathcal{B}(1)$ and $\mathcal{BB}(\lambda)$ are independent because $\cov[\mathcal{B}(1),\mathcal{BB}(\lambda)] = 0$ by construction. \hfill$\square$
 

==> old/prop1_old.tex <==
\renewcommand{\thelemma}{A.1}
\begin{lemma}\label{lemS0} For a given $\tau \in (0,1)$ and $h^2(\tau) \coloneqq 1/(\tau(1-\tau))$
\[
 h(\tau){\sf J}^{-1/2}S_n(\lambda,\tau,\beta_0(\tau)) \Rightarrow {\cal B}_m(\lambda)+  h(\tau){\sf J}^{-1/2}{\sf H} R\left(\lambda  \Delta(\tau)+\delta(\tau) \int_0^\lambda g(v){\sf d}v\right).
 \]    
\end{lemma}

\input{proofs/lemA1}


\textbf{Proof of Proposition \ref{prop_fixtau}.}  Recall that $\tilde\beta_{2,n}(\tau)$ denotes a solution to the constrained optimization defined in Eq.\ \eqref{eq:beta_tilde} (i.e. assuming $\beta_{1}(\tau) = 0$).  Moreover, set
\[
\bar R  \coloneqq \begin{bmatrix}
    0_{p \times k} \\  I_k
\end{bmatrix},
\]
so that, under the null, 
\[
\bar R\beta_{2,0}(\tau) = \beta_0(\tau) = \begin{bmatrix}
    0_p \\ \beta_{2,0}(\tau)
\end{bmatrix}.
\]

Next, using the same argument that lead to Eq.\ \eqref{eq:decA1}, we get
\begin{align*}
S_n(\lambda,\tau,\tilde\beta_n(\tau))=  S_n(\lambda,&\tau,\beta_0(\tau)) \\
\,&  + \frac{1}{\sqrt{n}}\sum_{i=1}^{\floor{\lambda n}}x_i(F_i(x_{2,i}'\tilde\beta_{2,n}(\tau)-F_i(x_{2,i}'\tilde\beta_{2,0})) + o_p(1)\\
\stackrel{(1)}{=} \,& S_n(\lambda,\tau,\beta_0(\tau)) \\
\,&  + \frac{1}{n}\sum_{i=1}^{\floor{\lambda n}}x_ix_{2,i}' f_i(x_{2,i}'\beta_{2,0}(\tau))\sqrt{n}(\beta_{2,n}(\tau)-\beta_{2,0}(\tau)) + o_p(1)\\
\stackrel{(2)}{=} \,& S_n(\lambda,\tau,\beta_0(\tau)) \\
\,&  + \frac{1}{n}\sum_{i=1}^{\floor{\lambda n}}x_ix_i'f_i(x_i'\beta_0(\tau)) (\bar R \sqrt{n}(\tilde\beta_{2,n}(\tau)-\beta_{2,0}(\tau)))  + o_p(1) \\
\stackrel{(3)}{=} \,& S_n(\lambda,\tau,\beta_0(\tau))   +  \lambda{\sf H}\sqrt{n}(\tilde\beta_n(\tau)-\beta_0(\tau)) + o_p(1),
% (0,\tilde\beta_{2,n}'(\tau))', 
\end{align*}
where $\tilde\beta_n(\tau) = \bar R\tilde\beta_{2,n}(\tau) = (0_p',\tilde\beta_{2,n}'(\tau))'$ and (1) uses first order Taylor-series expansion (see \citealp[proof of lem. 1]{qu:2008}), (2) is due to $x_ix_i'R = x_ix_{2,i}'$, and (3) is due to Ass.\ \ref{ass:C} that also defines the $m \times m$ matrix {\sf H}. Moreover, let ${\sf H}_{ij}$ and ${\sf J}_{ij}$, $i,j \in \{1,2\}$, denote the $ij$-th block of {\sf H} and {\sf J}, respectively, and partition 
\[
S_n(\lambda,\tau,t) = (S_{1,n}(\lambda,\tau,t_1)',S_{2,n}(\lambda,\tau,t_2)')'
\]
to conform with the partitioning $\beta_0(\tau) = (\beta_{1,0}(\tau)',\beta_{2,0}(\tau)')'$. Then,
\[
\sqrt{n}(\tilde\beta_n(\tau)-\beta_0(\tau)) = -\begin{bmatrix} 0_p \\ {\sf H}_{22}^{-1}S_{n,2}(1,\tau,\beta_{2,0}(\tau)) \end{bmatrix} + o_p(1),
\]
see also \citet[Proof of Thm. 1]{koemach:99} for the partitioning. Next, note that (see, e.g., \citealp[Proof of Prop. 1]{qu:2008})
\[
(\tau(1-\tau){\sf J})^{-1/2}S_{n}(\lambda,\tau,\beta_0(\tau))  \Rightarrow {\cal B}_{m}(\lambda) 
\]
and
\begin{align*}
    (\tau(1-\tau){\sf J}_{22})^{-1/2}&S_{2,n}(\lambda,\tau,\beta_0(\tau))  \\
    = & (\tau(1-\tau){\sf J}_{22})^{-1/2}\frac{1}{\sqrt{n}}\sum_{i=1}^{\floor{\lambda n}} x_{2,i}\psi_{\tau}(y_i-x_{2,i}'\beta_{2,0}(\tau))  \Rightarrow {\cal B}_k(\lambda). 
\end{align*}
Moreover, 
\begin{align*}
  &\begin{bmatrix} 0_p \\ {\sf H}_{22}^{-1}S_{n,2}(1,\tau,\beta_0(\tau)) \end{bmatrix}  \\
 & \quad \quad = \begin{bmatrix} 0_{p \times p} & 0_{p \times k} \\  0_{k \times p} & {\sf H}_{22}^{-1}({\sf J}_{22}^{-1/2})^{-1} \end{bmatrix} \begin{bmatrix} 0_p \\ {\sf J}_{22}^{-1/2}S_{2,n}(1,\tau,\beta_0(\tau)) \end{bmatrix} \\
 & \quad \quad = \begin{bmatrix} 0_{p \times p} & 0_{p \times k} \\  0_{k \times p} & {\sf H}_{22}^{-1}({\sf J}_{22}^{-1/2})^{-1} \end{bmatrix} {\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau)) \eqqcolon A {\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau)),
\end{align*}
say, where the $m \times m$ matrix $A$ has been implicitly defined. Hence, for $\bar M \coloneqq I_m-M$
\begin{align*}
    H_n(\lambda,\tau,\tilde\beta(\tau)) = \,& {\sf J}^{-1/2}S_n(\lambda,\tau,\beta_0(\tau)) - \lambda {\sf J}^{-1/2}{\sf H}A{\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau)) + o_p(1)    \\
    =\,&{\sf J}^{-1/2}S_n(\lambda,\tau,\beta_0(\tau))-\lambda (I-M){\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau))  \\
     \,&  \qquad\qquad\qquad-\lambda M {\sf J}^{-1/2}{\sf H}A{\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau)) + o_p(1).
\end{align*}

For
\begin{align}
    \bar{R} \coloneqq \begin{bmatrix} I_p \\ 0_{k\times p} \end{bmatrix}
\end{align}
we get by Lemma \ref{lemS0}
\begin{align*}
  \bar R'\tilde H_n(\lambda,\tau,\tilde\beta(\tau)  \Rightarrow  {\cal B}{\cal B}_p(\lambda) + \delta(\tau)\bar R'{\sf J}^{-1/2}{\sf H}\bar{R}\left((1-\lambda)\int_0^\lambda g(v){\sf d}v  -\lambda \int_\lambda^1 g(v){\sf d}v\right).
\end{align*}

Moreover, if $\lambda = 1$
\begin{align*}
  H_n(1,\tau,\tilde\beta(\tau)) = \,& (M-B){\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau)) + o_p(1) \\
\Rightarrow \,&\begin{bmatrix}
    {\cal B}_p(1) \\ 0_k
\end{bmatrix} +
\begin{bmatrix}
    \bar R'{\sf J}^{-1/2}{\sf H}\bar{R}(\Delta(\tau)-\delta(\tau)\int_0^1g(v){\sf d}v) \\ 0_k
\end{bmatrix}  
\end{align*}

 

\begin{align*}
    (I-M){\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau)) = \,& \begin{bmatrix} 0_p \\ {\sf J}_{22}^{-1/2}S_{n,2}(1,\tau,\beta_0(\tau)) \end{bmatrix}  \\
    M {\sf J}^{-1/2}{\sf H}A{\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau))  = \,&\begin{bmatrix} \bar R' {\sf J}^{-1/2}{\sf H}A{\sf J}^{-1/2}R {\sf J}_{22}^{-1/2}S_{n,2}(1,\tau,\beta_0(\tau))\\ 0_k \end{bmatrix}
\end{align*}

\rd (Under homoskedasticity, ${\sf J}^{-1/2}{\sf H}A = I_m - M$.)\bk  


The matrix, ${\sf J}^{-1/2}{\sf H}A$ is idempotent of rank $k$ with ${\sf diag}({\sf J}^{-1/2}{\sf H}A)=(0_p',1_k')'$. 


Hence, for $\tilde H_n$ defined in Eq.\ \eqref{eq:Htilde}, we get
\begin{align*}
(\tau(1-\tau)&)^{-1/2}\tilde H_n(\lambda,\tau,\tilde\beta(\tau)) \\
\, & = (\tau(1-\tau))^{-1/2}({\sf J}^{-1/2}S_n(\lambda,\tau,\beta_0(\tau))-\lambda {\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau))) + o_p(1) \\
\, & \Rightarrow {\mathcal B\cal B}_m(\lambda).
\end{align*}
If $\lambda = 1$, then
\begin{equation}
\begin{split}
    H_n(1,\tau,\tilde\beta(\tau)) = \,& M{\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau)) \\
    \,& \qquad\qquad - M{\sf J}^{-1/2}{\sf H}A {\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau)) + o_p(1) \\
    = \,& (M- B){\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau)) + o_p(1),
\end{split}
\end{equation}
where $B \coloneqq M{\sf J}^{-1/2}{\sf H}A$ is a $m \times m$ nilpotent matrix (i.e. $B^{j} = 0_{m \times m}$, $j > 1$)  with $MB' = 0_{m \times m}$, and $M-B$ is idempotent of rank $p$ (recall the definition of $M$, cf. Eq.\ \eqref{eq:Mmatrix}). Therefore, 
\[
(\tau(1-\tau))^{-1/2}H_n(1,\tau,\tilde\beta(\tau)) \rightarrow_d {\mathcal B}_p(1).
\]

\rd Because (only if ${\sf J} = {\sf H}$ up to a scalar; i.e. homoskedasticitiy), 
\[
{\sf J}^{-1/2}{\sf H} \begin{bmatrix} 0_{p \times p} & 0_{p \times k} \\  0_{k \times p} & {\sf H}_{22}^{-1}({\sf J}_{22}^{-1/2})^{-1} \end{bmatrix} =\begin{bmatrix} 0_{p \times p} & 0_{p \times k} \\  0_{k \times p} & I_k \end{bmatrix}
\]
the claim follows immediately from the construction of $H_n(\lambda,\tau,t)$ (cf. Eq.\ \eqref{eq:Hn}) and Ass.\ \ref{ass:C}. \bk

\hfill$\square$

% {\bf Sketches} Let $\bar M \coloneqq I_m-M$. In a first step, let me show that
% \begin{equation}
% \begin{split}
%     H_n(\lambda,\tau,\tilde\beta(\tau)) = \,& (I_m - \lambda \bar M){\sf J}^{-1/2}S_n(\lambda,\tau,\beta_0(\tau)) \\
%     \,& \qquad\qquad -\lambda (I_m -  \bar M){\sf J}^{-1/2}{\sf H}\Xi {\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau)) + o_p(1), 
% \end{split}
% \end{equation}
% where
% \[
% \Xi \coloneqq \begin{bmatrix} 0_{p \times p} & 0_{p \times k} \\  0_{k \times p} & {\sf H}_{22}^{-1}({\sf J}_{22}^{-1/2})^{-1} \end{bmatrix}
% \]


\textbf{Proof of Corollary \ref{cor1}.} By Proposition \ref{prop1},
$\tilde H_n(\lambda,\tau,\tilde\beta_n(\tau))\Rightarrow \sqrt{\tau(1-\tau)} {\cal{BB}}_{m}(\lambda),$ so that
\[
\tilde H_n(\lambda,\tau,\tilde\beta_n(\tau))M \Rightarrow \sqrt{\tau(1-\tau)}\begin{bmatrix} {\mathcal{BB}_p}(\lambda) \\ 0_k \end{bmatrix},
\]
and, because $\mathcal{BB}(1)=0$,
\[
H_n(1,\tau,\tilde\beta_n(\tau)) \Rightarrow \sqrt{\tau(1-\tau)}\begin{bmatrix} {\mathcal{B}_p}(1) \\ 0_k \end{bmatrix}
\]
The claim follows from the continuous mapping theorem noting that $\mathcal{B}(1)$ and $\mathcal{BB}(\lambda)$ are independent because $\cov[\mathcal{B}(1),\mathcal{BB}(\lambda)] = 0$ by construction. \hfill$\square$
 

==> old/teststat_old.tex <==
Consider the following sequential process based on the subgradient of the unconstrained quantile regression 
\begin{align}\label{eq:S_process}
S_{n}(\lambda,\tau,t) \coloneqq n^{-1/2}\sum_{i=1}^{\floor{\lambda n}}x_i\psi_\tau(y_i - x_i't), \quad t \in \mathbb{R}^{m},
\end{align}
where $\lambda \in [0,1]$ indexes the time fraction, and $\psi_\tau(u) \coloneqq 1\{u \leq 0\}-\tau$. Moreover, introduce the (constrained) estimator $\tilde\beta_n(\tau) \coloneqq \left(0, \alpha_{n}(\tau)'\right)'$, where
    \begin{align}\label{eq:beta_tilde}
    \alpha_{n}(\tau) \coloneqq \argmin\limits_{\alpha \in \mathbb{R}^k} \sum_{i=1}^n\rho_{\tau}(y_i-w_{i}'\alpha),
    \end{align}
% \quad \rho_\tau(u) \coloneqq u(1\{u\leq0\}-\tau).
% Comment: These equations are "crowded"; I suggest
% removing the definitions of these functions from the
% equations to make them cleaner.
where $\rho_\tau(u) \coloneqq u(1\{u\leq0\}-\tau)$. Our tests \bk are \bk based on the following process
\begin{equation}\label{eq:Hn}
H_n(\lambda,\tau,t) \coloneqq (X_n'X_n/n)^{-1/2}S_n(\lambda,\tau,t),\quad \lambda,\tau \in [0,1],\;t \in \mathbb{R}^m,
\end{equation}
where $X_n \coloneqq (x_1',\dots,x_n')'$ is $n \times m$. As pointed out by \cite{qu:2008}, the process in\ \eqref{eq:Hn} is asymptotically pivotal when evaluated at the true parameter vector; see also \cite{parzen:94} for a similar argument. This allows us to construct tests that do not require trimming over time.

The main idea behind our test statistic is to combine two detectors that are respectively designed to find deviations from $H_{0,1}$ and $H_{0,2}$. More specifically, a CUSUM-type statistic 
$${\sf LM_1}(\lambda,\tau) \coloneqq \left\Vert \Delta H_n(\lambda,\tau,\tilde\beta_n(\tau)) \right\Vert_\infty,$$
with
$$
\Delta H_n(\lambda,\tau,\tilde\beta_n(\tau)) \coloneqq H_n(\lambda,\tau,\tilde\beta_n(\tau))-\lambda  H_n(1,\tau,\tilde\beta_n(\tau))
$$
\bk is \bk used to test $H_{0,1}$, while the restriction of $H_{0,2}$ is verified using the LM (Lagrange Multiplier) statistic
$$ {\sf LM_2}(\tau) \coloneqq \left\Vert H_n(1,\tau,\tilde\beta_n(\tau)) \right\Vert_\infty.$$
Since ${\sf LM}_1$ has no power against constant deviations from the null, \bk and \bk ${\sf LM}_2$ lacks power if Granger causality is unstable, our tests will be of the form 
\begin{equation}\label{psi}
\varphi\big({\sf LM_1}+{\sf LM_2}\big),
\end{equation}
for some weighting function $\varphi: [0,1] \times [0,1] \mapsto \mathbb{R}$ specified below.

In what follows, we distinguish between situations where our interest lies in detecting deviations from the null ($i$) at a given quantile or ($ii$) across various quantiles. \bk To \bk derive the properties of theses tests, we impose the following assumptions that are similar to those in \cite{qu:2008} and \cite{oka:11}.

\renewcommand{\theassumption}{A}
\begin{assumption}\label{ass:A} Let $u_{i,n}(\tau) \coloneqq y_i-\beta_{i,n}(\tau)'x_i$. Then $1\{u_i(\tau)\leq 0\}-\tau$ is a martingale difference array with respect to $\mathcal F_{i-1}\coloneqq \sigma(\{y_{j-1},x_j: j \leq i\})$ for any $\tau \in [0,1]$.
\end{assumption}

Let $f_i(\cdot)$, $F_i(\cdot)$ and $F^{-1}_i(\cdot)$ denote the conditional density, conditional distribution, and conditional quantile function, respectively, of $y_i$ given $w_i$.

\renewcommand{\theassumption}{B}
\begin{assumption}\label{ass:B} 
\textcolor[rgb]{1,1,1}{.}
\begin{enumerate}[label=\textnormal{\textbf{B.\arabic*}},ref=B.\arabic*]
    \item The distribution functions $F_i(\cdot)$ are absolutely continuous, with continuous densities $f_i(\cdot)$ satisfying $0 < \ubar{u} \leq f_i(F^{-1}_i(\tau)) \leq \bar{u} < \infty$ for all $i$.
    \item For any $\epsilon > 0$, there exists a $\sigma(\epsilon) > 0$ such that
$|f_i(F^{-1}_i(\tau)+s)-f_i(F^{-1}_i(\tau))| \leq \epsilon$ for all $|s| < \sigma(\epsilon)$ and all $1 \leq i \leq n$.
\end{enumerate}
\end{assumption}

\renewcommand{\theassumption}{C}
\begin{assumption}\label{ass:C} 
The regressors are assumed to satisfy: 
\textcolor[rgb]{1,1,1}{.}
\begin{enumerate}[label=\textnormal{\textbf{C.\arabic*}},ref=B.\arabic*]
    \item The vector $w$ contains a constant.
\item  $\plim_{n \rightarrow \infty} \frac{1}{n}\sum_{i=1}^{\floor{\lambda n}}f_i(F^{-1}_i(\tau))x_ix_i' = \lambda {\sf H}(\tau)$ uniformly in $\lambda \in [0,1]$, where ${\sf H}(\tau)$ is a $m \times m$ non-random positive definite matrix.
\item There exists $a > 0$ and $A<\infty$ such that $\Ex[\left\Vert x_i\right\Vert^{4+a}] \leq A$.  
\item There exists $b > 0$ and $B<\infty$ such that for any $n$:
$$\frac{1}{n}\sum_{i=1}^n\Ex[\left\Vert x_i\right\Vert^{3(1+b)}] \vee \Ex[\frac{1}{n}\sum_{i=1}^n\left\Vert x_i\right\Vert^{3}]^{1+b} \leq B.$$
\item $\plim_{n \rightarrow \infty} \frac{1}{n} \sum_{i=1}^{\floor{\lambda n}}x_ix_i' = \lambda {\sf J}$ uniformly in $\lambda \in [0,1]$, where ${\sf J}$ is a $m \times m$ non-random positive definite matrix.
\end{enumerate}
\end{assumption}

\bk These \bk assumptions are standard in the context of tests for structural breaks in quantile models and of tests for Granger causality in quantiles. Assumption \ref{ass:A} restricts the dependence over time. Serial independence is not required, instead we have a martingale difference assumption on the innovations. Assumption \ref{ass:B} introduces positivity and smoothness assumptions on the conditional density of $y_i$ given $x_i$. Assumption C imposes restrictions on the regressors $x_i$, in particular on the existence of moments. This assumption rules out trends in the regressors, but \bk it \bk allows for heteroscedasticity.

\subsection{Granger Causality at a Given Quantile}

Let $\beta_0(\tau) \coloneqq (0_p',\alpha_{0}(\tau)')'$ be the true coefficient under the null, define
\begin{align}
    R \coloneqq \begin{bmatrix} I_p \\ 0_{k\times p} \end{bmatrix}, \quad \bar R \coloneqq \begin{bmatrix} 0_{p\times k} \\ I_{k} \end{bmatrix},
\end{align}
and set ${\sf C}(\tau) \coloneqq {\sf J}^{-1/2}{\sf H}(\tau).$ Note that ${\sf C}(\tau)$ is a square root of the inverse of the variance-covariance matrix of the limiting distribution of the estimator that solves the unrestricted quantile regression problem (\citealp{koenker:05}). Moreover, let ${\sf H}_{\alpha}(\tau)$ and ${\sf J}_{\alpha}$, denote the lower-right $k \times k$ block of {\sf H}$(\tau)$ and {\sf J}, respectively, and partition 
\[
S_n(\lambda,\tau,t) = (S_{n,\gamma}(\lambda,\tau,t_\gamma)',S_{n,\alpha}(\lambda,\tau,t_\alpha)')', \quad t_\gamma \in \mathbb{R}^p,\;t_\alpha \in \mathbb{R}^k
\]
to conform with the partitioning $\beta_0(\tau) = (\gamma_{0}(\tau)',\alpha_{0}(\tau)')'$ for $\gamma_0(\tau) = 0_p$.

\begin{proposition}\label{fixtau:prop1}
Assume that Assumptions \ref{ass:A}, \ref{ass:B}, and \ref{ass:C} hold. For a given $\tau \in {\cal T}$,  
\[
{\sf C}(\tau)\sqrt{n}(\tilde\beta_n(\tau)-\beta_0(\tau)) = -{\sf P}(\tau){\sf J}^{-1/2}S_{n}(1,\tau,\beta_{0}(\tau))  + o_p(1)
\]
for $P(\tau) \coloneqq {\sf C}(\tau) \bar R(\bar R'{\sf C}(\tau) \bar R)^{-1}\bar R'$. Moreover, it holds uniformly in $\lambda \in [0,1]$ 
\begin{align*}
H_n(\lambda,\tau,\tilde\beta_n(\tau))= {\sf J}^{-1/2}S_n(\lambda,\tau,\beta_0(\tau))- \lambda P(\tau){\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau)) + o_p(1),
\end{align*}
with
\[
 h(\tau){\sf J}^{-1/2}S_n(\lambda,\tau,\beta_0(\tau)) \Rightarrow {\cal B}_m(\lambda)+  h(\tau){\sf C}(\tau) R\left(\lambda  \Delta(\tau)+\delta(\tau) \int_0^\lambda g(v){\sf d}v\right).
 \]
 where $h^2(\tau) \coloneqq 1/(\tau(1-\tau))$. 
\end{proposition}

 
From the result above, we can directly deduce the limiting distribution of the two test statistics as summarized by Corollary \ref{corHtilde}.

\begin{corollary}\label{corHtilde} 
For a given $\tau \in {\cal T}$, it holds under the assumptions of Proposition \ref{fixtau:prop1} uniformly in $\lambda \in [0,1]$ 
\begin{align*}
  h(\tau)& R'\Delta H_n(\lambda,\tau,\tilde\beta_n(\tau))\\  &\Rightarrow  {\cal BB}_p(\lambda) + h(\tau)\delta(\tau) R'{\sf C}(\tau)R\left((1-\lambda)\int_0^\lambda g(v){\sf d}v  -\lambda \int_\lambda^1 g(v){\sf d}v\right) \eqqcolon {\cal Z}^{(1)}(\lambda,\tau) 
\end{align*}
and 
\begin{align*}
h(\tau)&R'H_n(1,\tau,\tilde\beta_n(\tau))\\ 
\,&\Rightarrow 
    \tilde {\cal B}_p(1,\tau) +
h(\tau)
    R'T(\tau){\sf C}(\tau)R\left(\Delta(\tau)+\delta(\tau)\int_0^1g(v){\sf d}v\right)  \eqqcolon {\cal Z}^{(2)}(\tau)
\end{align*}
where $\tilde{\cal B}_m(\lambda,\tau) \coloneqq T(\tau){\cal B}_m(\lambda)$, with $T(\tau)$ denoting the inverse of the $m \times m$ matrix of eigenvectors of $I-P(\tau)$.
\end{corollary}

Interestingly, and contrary to the corresponding GMM result in \cite{rossi:2005}, the limiting distribution of the LM statistic $H_n(1,\tau,\tilde\beta_n(\tau))$ is not pivotal because the projection matrix $P(\tau)$ is oblique (i.e. idempotent of rank $k$ but not symmetric). An important exception is given if the following additional condition is satisfied: 
 
\renewcommand{\theassumption}{D}
\begin{assumption}\label{ass:D}  The  $p \times k$ matrix $Q(\tau) \coloneqq R'{\sf C}(\tau)\bar R {\sf H}^{-1}_{\alpha}(\tau){\sf J}^{1/2}_{\alpha}$ is zero, where ${\sf H}_{\alpha}(\tau)$ and ${\sf J}_{\alpha}$ denote the lower-right $k \times k$ sub-matrix of ${\sf H}(\tau)$ and {\sf J}, respectively, partitioned according the $k \times 1$ subvector $\alpha(\tau)$ of $\beta(\tau) = (\gamma(\tau)', \alpha(\tau)')'$.
\end{assumption}
 
Assumption\ \ref{ass:D} ensures that the oblique projection matrix $P(\tau)$ defined in Proposition\ \ref{fixtau:prop1} is equal to the orthogonal projection $\bar R(\bar R'\bar R)^{-1}\bar R' = \bar R\bar R'$, which follows from observing that $P(\tau)$ decomposes into an orthogonal projection perturbed by a nilpotent matrix
\begin{equation}\label{project}
P(\tau) = {\sf C}(\tau) \bar R(\bar R'{\sf C}(\tau) \bar R)^{-1}\bar R' = \bar R\bar R'  + \begin{bmatrix}
    0_{p\times p} & Q(\tau) \\ 0_{k\times p} & 0_{k\times k}
\end{bmatrix}.
\end{equation}
A sufficient condition for Assumption\ \ref{ass:D} is ${\sf H}c(\tau) = {\sf J}(\tau)$ for some scalar $c(\tau) \in (0,\infty)$, which holds under homoscedasticity. Alternatively, Assumption\ \ref{ass:D} is satisfied if $w$ is just a constant or, more generally, under conditional mean independence of $z$ with respect to $w$ (i.e. $\Ex[z \vert w] = \Ex[z]$) as both of theses conditions ensure under the null $Q(\tau) = 0_{p \times k}$. 


\begin{corollary}\label{corH0}   
Under the null hypothesis and Assumptions \ref{ass:A}--\ref{ass:D}, we get for a given $\tau \in {\cal T}$ and uniformly in $\lambda \in [0,1]$ 
\[
h(\tau)H_n(\tau,\lambda,\tilde\beta_n(\tau)) \Rightarrow \begin{bmatrix} {\mathcal B}_p(\lambda) \\ {\cal BB}_k(\lambda) \end{bmatrix},
\]
where ${\cal BB}_k(\cdot)$ and ${\cal B}_p(\cdot)$ are independent.
\end{corollary}

The $p$-dimensional Brownian motion ${\cal B}_p$ and the $k$-dimensional Brownian bridges ${\cal BB}_k$ arise due to the restricted and unrestricted components of the process tow-parameter process $H_n(\lambda,\tau,\beta(\tau))$, respectively. The limiting random variable under the null is independent of $\tau$. While this is true if Assumption\ \ref{ass:D} holds, violations from this assumption introduce dependence on nuisance parameters (cf. Proposition \ref{cor1}).

Based on the previous result, we will now introduce our first test statistic, suited to test $H_0$ at a given quantile $\tau$
\begin{align*}\label{eq:GCtest1}
   {\sf LM}(\tau) \coloneqq h(\tau)\left(\ssup\limits_{\lambda \in [0,1]}{\sf LM}_{1}(\lambda,\tau) + {\sf LM}_{2}(\tau)\right).
\end{align*}

For fixed $\tau$, the test statistic essentially consists of the sum of two individual test statistics, which reflect the two parts of the alternative hypothesis. Both statistics are based on the standardized subgradient of the unconstrained quantile regression through the process $H_n(\lambda,\tau,t)$ from \eqref{eq:Hn}. The first part, ${\sf LM}_{1}(\lambda,\tau)$, is the CUSUM part that detects structural breaks in the parameter $\gamma_i(\tau)$. Typically, for CUSUM statistics, one considers the supremum over the potential breakpoints $\lambda \in [0,1]$. The second part, ${\sf LM}_{2}(\tau)$, is essentially the LM  statistic for the hypothesis $H_{0,2}$.  
%which serves for detecting

Corollary \ref{corHtilde} states why it makes sense to consider the sum of the two individual test statistics: The first statistic does have local power against structural breaks, but it has no power if there is Granger causality with constant parameters. The second part has power if there is Granger causality with constant parameters, but it has no power if $\Delta(\tau) = 0$ and $\int_0^1g(v){\sf d}v = 0$. The interpretation of the latter would be that there are structural breaks that lie in opposite directions over time.

\begin{corollary}\label{cor1}
For a given $\tau \in {\cal T}$, we get under the assumptions of Proposition \ref{fixtau:prop1}
\[
{\sf LM}(\tau) \rightarrow_d 
\ssup\limits_{\lambda \in [0,1]} \left\Vert{\cal Z}^{(1)}(\lambda,\tau)\right\Vert_\infty+\left\Vert{\cal Z}^{(2)}(\tau)\right\Vert_\infty,
\]
while under the null
\[
{\sf LM}(\tau) \rightarrow_d 
\ssup\limits_{\lambda \in [0,1]} \left\Vert{\cal BB}_p(\lambda)\right\Vert_\infty+\left\Vert{\tilde{\cal B}}_p(1,\tau)\right\Vert_\infty.
\]
where ${\cal BB}_p$ and $\tilde {\cal B}_p(\lambda,\tau)$ are independent. If Assumption \ref{ass:D} holds, then $\tilde {\cal B}_p(\lambda,\tau) = {\cal B}_p(\lambda)$.
\end{corollary}

Thus, unless Assumption \ref{ass:D} is satisfied, the limiting distribution is not pivotal due to the second element ${\sf LM}_{2}$ of our test statistic that induces dependence on the quantile level $\tau$ via $Q(\tau)$. More specifically, it can be shown that
\[
{\sf LM}_{2}(\tau) = \left\Vert (I-P(\tau)){\sf J}^{-1/2}S_n(1,\tau,\beta_0(\tau))\right\Vert_\infty + o_p(1),
\]
where the oblique projection $P(\tau)$ causes quantile dependece because it cannot be diagonalized; cf. Eq.\ \eqref{project}. The distribution of ${\sf LM}_2$ can be viewed as a maximum of $p$-scaled absolute standard normals, where--similar to the discussion in \cite{hansen:21}--the scaling differs in general from unity, thereby capturing deviations from Assumption \ref{ass:D} (e.g. from homoskedasticity to heteroskedasticity).

\subsection{Granger Causality at all Quantiles}

To avoid multiple testing issues when performing inference across various quantiles, we extend the test statistics from the previous section to allow uniform inference across both $\lambda$ {\it and} $\tau$. Following \cite{andpol:1994} and  \cite{hansen:1996b}, we consider the following test statistics: 
\begin{equation}\label{eq:GCtest1}
\begin{split}
{sup\sf{LM}} \coloneqq \,&\ssup\limits_{\tau \in \cal T}\left(\ssup\limits_{\lambda \in [0,1]}{\sf LM}_{1}(\lambda,\tau) + {\sf LM}_{2}(\tau)\right), \\
   \textnormal{\it{exp}\sf{LM}} \coloneqq \,&\int_{\cal T}{\sf exp}\left[\frac{1}{2}\left(\ssup\limits_{\lambda \in [0,1]}{\sf LM}_{1}(\lambda,\tau) + {\sf LM}_{2}(\tau)\right)\right] d\tau. 
   \end{split}
\end{equation}
While both weighting schemes (over $\tau$) direct power against relatively distantly located alternatives, $\textnormal{\it{exp}\sf{LM}}$ can be considered optimal (see also \citealp{rossi:2005}).

Similar to Proposition \ref{fixtau:prop1}, we first derive the properties of the process Eq. \eqref{eq:Hn} that serves as the building block of our test statistics. 

% Since we need to derive weak convergence uniformly in both $\lambda$ {\it and} $\tau$, we have to impose an additional regularity condition:
 % \renewcommand{\theassumption}{E}
% \begin{assumption}\label{ass:E} There exists a constant $M$ such that for all $i$, $\Ex[(x_i'x_i)^2] \leq M \in (0,\infty)$.
% \end{assumption}
% As discussed in \citet[Sec. 4]{qu:2008}, Assumption \ref{ass:E}, needed to establish stochastic equicontinuity of the process in Eq.\ \eqref{eq:Hn}, can be relaxed in principle. Given Assumptions \ref{ass:A}-\ref{ass:C} and \ref{ass:E}, we are now able to establish weak convergence along the path of the sequence of local alternatives:

 
\begin{proposition}\label{prop2} Assume that Assumptions \ref{ass:A}, \ref{ass:B}, and \ref{ass:C} hold uniformly in $\tau$. Then, uniformly in $(\tau,\lambda) \in \mathcal{T} \times [0,1]$, we have
\begin{align*}
R'\Delta H_n(\lambda,\tau,\tilde\beta_n(\tau)) \Rightarrow  \,& {\cal SS}_p(\lambda,\tau) + \delta(\tau) R'{\sf C}(\tau)R\left((1-\lambda)\int_0^\lambda g(v){\sf d}v  -\lambda \int_\lambda^1 g(v){\sf d}v\right) \\
\,& \eqqcolon {\cal Y}^{(1)}(\lambda,\tau)
\end{align*}
and
\begin{align*}
R'H_n(1,\tau,\tilde\beta_n(\tau))  \Rightarrow 
    \widetilde{\cal S}_p(1,\tau) +
    R'T(\tau){\sf C}(\tau)R\left(\Delta(\tau)+\delta(\tau)\int_0^1g(v){\sf d}v\right)  \eqqcolon {\cal Y}^{(2)}(\tau), 
\end{align*}
where $\widetilde{\cal S}_m(\tau,\lambda) \coloneqq T(\tau){\cal S}_{m}(\tau,\lambda)$ for ${\cal S}_{m}(\lambda,\tau) \coloneqq ({\cal S}_{1m}(\lambda,\tau),\dots,{\cal S}_{mm}(\lambda,\tau))'$ is an $m \times 1$ vector of independent Gaussian processes with
\[
\cov[{\cal S}_{im}(\lambda_1,\tau_1),{\cal S}_{im}(\lambda_2,\tau_2)] = (\lambda_1 \wedge \lambda_2)(\tau_1 \wedge \tau_2 - \tau_1\tau_2)
\]
and ${\cal SS}_m(\lambda,\tau) \coloneqq {\cal S}_m(\lambda,\tau) - \lambda {\cal S}_m(1,\tau)$ so that
\[
\cov[{\cal SS}_{im}(\lambda_1,\tau_1),{\cal SS}_{im}(\lambda_2,\tau_2)] = (\lambda_1 \wedge \lambda_2-\lambda_1\lambda_2)(\tau_1 \wedge \tau_2 - \tau_1\tau_2).
\]
\end{proposition}

Again, the weak limit of $H_n(1,\tau,\tilde\beta(\tau))$ is affected by nuisance parameters unless Assumption \ref{ass:D} holds, in which case $\widetilde {\cal S}_p(\lambda,\tau) = {\cal S}_p(\lambda,\tau).$ Moreover, note that ${\cal S}(1,\tau) = {\cal B}(\tau)$, while the Gaussian process ${\cal SS}(\lambda,\tau)$ is also referred to as a Brownian pillow or a pinned Brownian sheet; see also \citet[Sec 4]{qu:2008}. From the above, the limiting distribution of the test statistics follows readily by the continuous mapping theorem:

\begin{corollary}\label{cor4}
Uniformly in $(\tau,\lambda) \in \mathcal{T} \times [0,1]$, we have under the conditions of Proposition \ref{prop2}
\begin{align*}
   {sup\sf{LM}} \rightarrow_d \,&\ssup\limits_{\tau \in \cal T}\left(\ssup\limits_{\lambda \in [0,1]} \left\Vert {\cal Y}^{(1)}(\lambda,\tau) \right\Vert_\infty + \left\Vert{\cal Y}^{(2)}(\lambda,\tau) \right\Vert_\infty\right),  \\
   \textnormal{\it{exp}\sf{LM}} \rightarrow_d \,&\int_{\cal T}{\sf exp}\left[\frac{1}{2}\left(\ssup\limits_{\lambda \in [0,1]}\left\Vert {\cal Y}^{(1)}(\lambda,\tau) \right\Vert_\infty + \left\Vert {\cal Y}^{(2)}(\lambda,\tau) \right\Vert_\infty\right)\right] d\tau, 
\end{align*}
while, under the null, ${\cal Y}^{(1)}(\lambda,\tau) = {\cal SS}_p(\lambda,\tau)$ and ${\cal Y}^{(2)}(\lambda,\tau) = \widetilde {\cal S}_p(1,\tau)$.  If Assumption \ref{ass:D} holds, then $\widetilde {\cal S}_p(\lambda,\tau) = {\cal S}_p(\lambda,\tau)$.
\end{corollary}







==> table.tex <==
\setlength{\tabcolsep}{4.66pt}
\begin{sidewaystable}[htbp]
\begin{center}\small
\begin{tabular}{rrccccccccccccccccccccc} \toprule \\[-.55cm]  \hline\\[-.4cm]
&&\multicolumn{4}{c}{{\sf size}} &&\multicolumn{4}{c}{{\sf power (A)}}&&\multicolumn{4}{c}{{\sf power (B)}}&&\multicolumn{4}{c}{{\sf power (C)}}\\
 \cmidrule(r){3-6}\cmidrule(r){8-11}\cmidrule(r){13-16}\cmidrule(r){18-21}
$n$&$\tau$&{\sf GC}&{\sf LM}&{\sf W0}&{\sf WB}&&{\sf GC}&{\sf LM}&{\sf W0}&{\sf WB}\\  \hline
250&0.05	&	0.047	&	0.058	&	0.089	&	0.050	&	&	0.087	&	0.096	&	0.127	&	0.077	&	&	0.064	&	0.079	&	0.101	&	0.062	&	&	0.190	&	0.214	&	0.272	&	0.193	\\
&0.10	&	0.041	&	0.048	&	0.069	&	0.055	&	&	0.094	&	0.104	&	0.096	&	0.082	&	&	0.056	&	0.065	&	0.084	&	0.061	&	&	0.252	&	0.273	&	0.306	&	0.256	\\
&0.15	&	0.047	&	0.052	&	0.047	&	0.050	&	&	0.087	&	0.097	&	0.096	&	0.092	&	&	0.069	&	0.073	&	0.074	&	0.070	&	&	0.311	&	0.333	&	0.334	&	0.307	\\
&0.20	&	0.048	&	0.055	&	0.037	&	0.054	&	&	0.098	&	0.107	&	0.090	&	0.101	&	&	0.073	&	0.079	&	0.066	&	0.078	&	&	0.349	&	0.376	&	0.336	&	0.347	\\
&0.25	&	0.042	&	0.045	&	0.029	&	0.047	&	&	0.104	&	0.113	&	0.074	&	0.099	&	&	0.072	&	0.081	&	0.062	&	0.071	&	&	0.391	&	0.408	&	0.340	&	0.370	\\
&0.30	&	0.056	&	0.059	&	0.029	&	0.055	&	&	0.104	&	0.112	&	0.081	&	0.113	&	&	0.074	&	0.081	&	0.054	&	0.085	&	&	0.414	&	0.427	&	0.342	&	0.409	\\
&0.35	&	0.053	&	0.058	&	0.031	&	0.057	&	&	0.106	&	0.115	&	0.073	&	0.113	&	&	0.085	&	0.092	&	0.052	&	0.082	&	&	0.426	&	0.447	&	0.321	&	0.421	\\
&0.40	&	0.048	&	0.053	&	0.029	&	0.059	&	&	0.116	&	0.126	&	0.068	&	0.117	&	&	0.086	&	0.095	&	0.045	&	0.092	&	&	0.448	&	0.460	&	0.331	&	0.435	\\
&0.45	&	0.042	&	0.047	&	0.023	&	0.047	&	&	0.120	&	0.129	&	0.060	&	0.110	&	&	0.081	&	0.091	&	0.041	&	0.087	&	&	0.445	&	0.470	&	0.321	&	0.445	\\
&0.50	&	0.043	&	0.048	&	0.021	&	0.055	&	&	0.106	&	0.116	&	0.057	&	0.117	&	&	0.081	&	0.088	&	0.040	&	0.091	&	&	0.445	&	0.463	&	0.318	&	0.435	\\
&0.55	&	0.049	&	0.054	&	0.022	&	0.057	&	&	0.115	&	0.124	&	0.060	&	0.117	&	&	0.083	&	0.089	&	0.041	&	0.084	&	&	0.441	&	0.463	&	0.313	&	0.423	\\
&0.60	&	0.056	&	0.061	&	0.023	&	0.058	&	&	0.108	&	0.119	&	0.061	&	0.117	&	&	0.084	&	0.089	&	0.046	&	0.087	&	&	0.427	&	0.452	&	0.315	&	0.413	\\
&0.65	&	0.052	&	0.061	&	0.023	&	0.055	&	&	0.106	&	0.114	&	0.070	&	0.111	&	&	0.080	&	0.087	&	0.050	&	0.083	&	&	0.401	&	0.429	&	0.349	&	0.421	\\
&0.70	&	0.052	&	0.059	&	0.029	&	0.058	&	&	0.102	&	0.114	&	0.078	&	0.116	&	&	0.083	&	0.091	&	0.058	&	0.084	&	&	0.394	&	0.420	&	0.343	&	0.398	\\
&0.75	&	0.051	&	0.054	&	0.036	&	0.055	&	&	0.098	&	0.105	&	0.091	&	0.105	&	&	0.071	&	0.082	&	0.069	&	0.084	&	&	0.366	&	0.391	&	0.343	&	0.378	\\
&0.80	&	0.049	&	0.054	&	0.042	&	0.048	&	&	0.091	&	0.101	&	0.087	&	0.100	&	&	0.078	&	0.088	&	0.068	&	0.079	&	&	0.349	&	0.375	&	0.331	&	0.344	\\
&0.85	&	0.049	&	0.057	&	0.055	&	0.052	&	&	0.087	&	0.097	&	0.097	&	0.098	&	&	0.077	&	0.085	&	0.087	&	0.081	&	&	0.301	&	0.326	&	0.321	&	0.312	\\
&0.90	&	0.046	&	0.053	&	0.072	&	0.051	&	&	0.082	&	0.096	&	0.102	&	0.091	&	&	0.070	&	0.081	&	0.103	&	0.080	&	&	0.235	&	0.264	&	0.296	&	0.264	\\
&0.95	&	0.048	&	0.052	&	0.096	&	0.058	&	&	0.066	&	0.082	&	0.144	&	0.084	&	&	0.057	&	0.065	&	0.123	&	0.073	&	&	0.161	&	0.191	&	0.279	&	0.199	\\
\cmidrule(r){3-6}\cmidrule(r){8-11}\cmidrule(r){13-16}\cmidrule(r){18-21}
&{\sf sup}	&	0.055	&	0.057	&	0.036	&	0.038	&	&	0.160	&	0.128	&	0.073	&	0.091	&	&	0.101	&	0.094	&	0.055	&	0.074	&	&	0.509	&	0.523	&	0.315	&	0.423	\\
&{\sf avg-exp}	&	0.055	&	0.055	&		&		&	&	0.196	&	0.149	&		&		&	&	0.117	&	0.105	&		&		&	&	0.567	&	0.584	&		&		\\
\hline\\[-.50cm]
\bottomrule
\end{tabular}
\end{center}
\end{sidewaystable}
